A Re-Parameterized Vision Transformer (ReVT) for Domain-Generalized Semantic Segmentation

The task of semantic segmentation requires a model to assign semantic labels to each pixel of an image. However, the performance of such models degrades when deployed in an unseen domain with different data distributions compared to the training domain. We present a new augmentation-driven approach to domain generalization for semantic segmentation using a re-parameterized vision transformer (ReVT) with weight averaging of multiple models after training. We evaluate our approach on several benchmark datasets and achieve state-of-the-art mIoU performance of 47.3% (prior art: 46.3%) for small models and of 50.1% (prior art: 47.8%) for midsized models on commonly used benchmark datasets. At the same time, our method requires fewer parameters and reaches a higher frame rate than the best prior art. It is also easy to implement and, unlike network ensembles, does not add any computational complexity during inference.

==> alg/tu_bs_colors.tex <==
\definecolor{tu0}{rgb}{0.7451, 0.1176, 0.2353}

\definecolor{tu1}{rgb}{1.0000, 0.8039, 0.0000}
\definecolor{tu11}{rgb}{1.0000, 0.8627, 0.3020}
\definecolor{tu12}{rgb}{1.0000, 0.9020, 0.4980}
\definecolor{tu13}{rgb}{1.0000, 0.9412, 0.6980}
\definecolor{tu14}{rgb}{1.0000, 0.9608, 0.8000}

\definecolor{tu2}{rgb}{0.9804, 0.4314, 0.0000}
\definecolor{tu21}{rgb}{0.9882, 0.6039, 0.3020}
\definecolor{tu22}{rgb}{0.9882, 0.7137, 0.4980}
\definecolor{tu23}{rgb}{0.9922, 0.8275, 0.6980}
\definecolor{tu24}{rgb}{0.9961, 0.8863, 0.8000}

\definecolor{tu3}{rgb}{0.6902, 0.0000, 0.2745}
\definecolor{tu31}{rgb}{0.7529, 0.2000, 0.4196}
\definecolor{tu32}{rgb}{0.8431, 0.4980, 0.6353}
\definecolor{tu33}{rgb}{0.9216, 0.7490, 0.8196}
\definecolor{tu34}{rgb}{0.9529, 0.8510, 0.8902}

\definecolor{tu4}{rgb}{0.4863, 0.8039, 0.9020}
\definecolor{tu41}{rgb}{0.6431, 0.8627, 0.9333}
\definecolor{tu42}{rgb}{0.7412, 0.9020, 0.9490}
\definecolor{tu43}{rgb}{0.8431, 0.9412, 0.9686}
\definecolor{tu44}{rgb}{0.8980, 0.9608, 0.9804}

\definecolor{tu5}{rgb}{0.0000, 0.5020, 0.7059}
\definecolor{tu51}{rgb}{0.3020, 0.6510, 0.7961}
\definecolor{tu52}{rgb}{0.5490, 0.7765, 0.8667}
\definecolor{tu53}{rgb}{0.7490, 0.8745, 0.9255}
\definecolor{tu54}{rgb}{0.8510, 0.9255, 0.9569}

\definecolor{tu6}{rgb}{0.0000, 0.3255, 0.4549}
\definecolor{tu61}{rgb}{0.2510, 0.4941, 0.5922}
\definecolor{tu62}{rgb}{0.5490, 0.6941, 0.7529}
\definecolor{tu63}{rgb}{0.7490, 0.8314, 0.8627}
\definecolor{tu64}{rgb}{0.8510, 0.8980, 0.9176}

\definecolor{tu7}{rgb}{0.0314, 0.0314, 0.0314}
\definecolor{tu71}{rgb}{0.3725, 0.3725, 0.3725}
\definecolor{tu72}{rgb}{0.5882, 0.5882, 0.5882}
\definecolor{tu73}{rgb}{0.7529, 0.7529, 0.7529}
\definecolor{tu74}{rgb}{0.8667, 0.8667, 0.8667}

\definecolor{tu8}{rgb}{0.7765, 0.9333, 0.0000}
\definecolor{tu81}{rgb}{0.8431, 0.9529, 0.3020}
\definecolor{tu82}{rgb}{0.8863, 0.9647, 0.4980}
\definecolor{tu83}{rgb}{0.9333, 0.9804, 0.6980}
\definecolor{tu84}{rgb}{0.9569, 0.9882, 0.8000}

\definecolor{tu9}{rgb}{0.5373, 0.6431, 0.0000}
\definecolor{tu91}{rgb}{0.6784, 0.7490, 0.3020}
\definecolor{tu92}{rgb}{0.7686, 0.8196, 0.4980}
\definecolor{tu93}{rgb}{0.8588, 0.8941, 0.6980}
\definecolor{tu94}{rgb}{0.9059, 0.9294, 0.8000}

\definecolor{tu10}{rgb}{0.0000, 0.4431, 0.3373}
\definecolor{tu101}{rgb}{0.3020, 0.6118, 0.5373}
\definecolor{tu102}{rgb}{0.5490, 0.7490, 0.7020}
\definecolor{tu103}{rgb}{0.7490, 0.8588, 0.8353}
\definecolor{tu104}{rgb}{0.8549, 0.9176, 0.9059}

\definecolor{tu110}{rgb}{0.8000, 0.0000, 0.6000}
\definecolor{tu111}{rgb}{0.8706, 0.3490, 0.7412}
\definecolor{tu112}{rgb}{0.9216, 0.6000, 0.8392}
\definecolor{tu113}{rgb}{0.9608, 0.8000, 0.9216}
\definecolor{tu114}{rgb}{0.9804, 0.8980, 0.9608}

\definecolor{tu120}{rgb}{0.4627, 0.0000, 0.4627}
\definecolor{tu121}{rgb}{0.5961, 0.2510, 0.5961}
\definecolor{tu122}{rgb}{0.7294, 0.4980, 0.7294}
\definecolor{tu123}{rgb}{0.8392, 0.6980, 0.8392}
\definecolor{tu124}{rgb}{0.9216, 0.8510, 0.9216}

\definecolor{tu130}{rgb}{0.4627, 0.0000, 0.3294}
\definecolor{tu131}{rgb}{0.6118, 0.3020, 0.5333}
\definecolor{tu132}{rgb}{0.7569, 0.5490, 0.6980}
\definecolor{tu133}{rgb}{0.8667, 0.7490, 0.8314}
\definecolor{tu134}{rgb}{0.9216, 0.8510, 0.9020}

==> tab/mathematical_formulations.tex <==
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\src}[0]{{\mathcal{D}^S}}
\newcommand{\tgt}[0]{{\mathcal{D}^T}}

\newcommand{\network}[1]{{\texttt{#1}}}

\newcommand{\mv}{\_\_.\_}

%DATASETS
\newcommand{\datatrain}[0]{{\mathcal{D}_\mathrm{train}}}
\newcommand{\datafull}[0]{{\mathcal{D}_\mathrm{full}}}
\newcommand{\dataval}[0]{{\mathcal{D}_\mathrm{val}}}
\newcommand{\datatest}[0]{{\mathcal{D}_\mathrm{test}}}
\newcommand{\datavalstar}[0]{{\mathcal{D}_\mathrm{val*}}}
\newcommand{\datateststar}[0]{{\mathcal{D}_\mathrm{test*}}}
\newcommand{\datadev}[0]{{\mathcal{D}_\mathrm{dev}}}
\newcommand{\dataooddev}[0]{{\mathcal{D}^\mathrm{OOD}_\mathrm{dev}}}
\newcommand{\databench}[0]{{\mathcal{D}_\mathrm{BM}}}

\newcommand{\cstrain}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{train}}}
\newcommand{\csval}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{val}}}
\newcommand{\cstest}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{test}}}
\newcommand{\csvalstar}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{val*}}}
\newcommand{\csteststar}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{test*}}}
\newcommand{\csdev}[0]{{\mathcal{D}^\mathrm{CS}_\mathrm{dev}}}

\newcommand{\bddtrain}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{train}}}
\newcommand{\bddval}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{val}}}
\newcommand{\bddtest}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{test}}}
\newcommand{\bddvalstar}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{val*}}}
\newcommand{\bddteststar}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{test*}}}
\newcommand{\bdddev}[0]{{\mathcal{D}^\mathrm{BDD}_\mathrm{dev}}}

\newcommand{\mvtrain}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{train}}}
\newcommand{\mvval}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{val}}}
\newcommand{\mvtest}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{test}}}
\newcommand{\mvvalstar}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{val*}}}
\newcommand{\mvteststar}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{test*}}}
\newcommand{\mvdev}[0]{{\mathcal{D}^\mathrm{MV}_\mathrm{dev}}}

\newcommand{\acdctrain}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{train}}}
\newcommand{\acdcval}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{val}}}
\newcommand{\acdctest}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{test}}}
\newcommand{\acdcvalstar}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{val*}}}
\newcommand{\acdcteststar}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{test*}}}
\newcommand{\acdcdev}[0]{{\mathcal{D}^\mathrm{ACDC}_\mathrm{dev}}}

\newcommand{\kittitrain}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{train}}}
\newcommand{\kittival}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{val}}}
\newcommand{\kittitest}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{test}}}
\newcommand{\kittivalstar}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{val*}}}
\newcommand{\kittiteststar}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{test*}}}
\newcommand{\kittidev}[0]{{\mathcal{D}^\mathrm{KIT}_\mathrm{dev}}}

\newcommand{\gtavfull}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{full}}}
\newcommand{\gtavtrain}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{train}}}
\newcommand{\gtavval}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{val}}}
\newcommand{\gtavtest}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{test}}}
\newcommand{\gtavvalstar}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{val*}}}
\newcommand{\gtavteststar}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{test*}}}
\newcommand{\gtavdev}[0]{{\mathcal{D}^\mathrm{GTA5}_\mathrm{dev}}}

\newcommand{\synthiafull}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{full}}}
\newcommand{\synthiatrain}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{train}}}
\newcommand{\synthiaval}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{val}}}
\newcommand{\synthiatest}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{test}}}
\newcommand{\synthiavalstar}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{val*}}}
\newcommand{\synthiateststar}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{test*}}}
\newcommand{\synthiadev}[0]{{\mathcal{D}^\mathrm{SYN}_\mathrm{dev}}}

==> tab/mathmacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematische Macros
%
% Mathematical macros for lectures and publications
%
% (c) Prof. Dr.-Ing. Tim Fingscheidt
%     IfN / TU Braunschweig, 2006-04-30
%




\newcommand{\nomathindent}{\hspace*{-10mm}}


% Mathematische Zeichen: -------------------------------------------------------
\newcommand{\entspricht}{\widehat{=}}
\newcommand{\folgerung}{\item[$\Rightarrow$]}
\newcommand{\lift}[1]{\raisebox{1.5ex}[-1.5ex]{#1}}
\newcommand{\ld}{\log_2}
\newcommand{\sign}{{\rm sign}}
\newcommand{\erfc}{{\rm erfc}}
\newcommand{\SNRSEG}{\mathrm{SNR}_{\mathrm{seg}}}
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\ERLEu}{\mathrm{ERLE}_u}
\newcommand{\ERLEd}{\mathrm{ERLE}_d}
%\newcommand{\conv}{\ast}
\newcommand{\conv}[1][]{\ast_{_{#1}}}
\newcommand{\circconv}{\otimes}
\newcommand{\class}{\mathrm{class}}
\newcommand{\Res}[1]{{\rm Res}\{#1\}}   % Residuum
\newcommand{\E}[1]{{\mathrm{E}}\{#1\}}  % Expectation
\newcommand{\Elr}[1]{{\mathrm{E}}\left\{#1\right\}}  % Expectation
%\newcommand{\unit}[1]{{\sf #1}}
\newcommand{\OK}{\mathbf{\sqrt{}}}
\newcommand{\QUANT}[1]{{\bf Q[}#1{\bf ]}}         % Quantisierungsfunktion
\newcommand{\Dist}{{\mathfrak{D}}}
\newcommand{\WER}{\mathrm{WER}}         % WER = Word error rate
\newcommand{\WRR}{\mathrm{WRR}}         % 1-WER = Word recognition rate
\newcommand{\ACC}{\mathrm{ACC}}         % Accuracy
\newcommand{\SER}{\mathrm{SER}}         % Sentence error rate
\newcommand{\PCorr}{\mathrm{PCorr}}     % = (1-(D+S)/R) *100%, used in htk
\newcommand{\PAcc}{\mathrm{PAcc}}       % = (1-WER) *100%, used in htk
\newcommand{\WA}{\mathrm{WA}}           % Word accuracy
\newcommand{\SA}{\mathrm{SA}}           % Sentence accuracy
\newcommand{\CS}{\mathrm{CS}}           % Confidence score
\newcommand{\LOGE}{\mathrm{logE}}       % logE parameter

% SPECOM lecture:
\newcommand{\AKF}[2][]{\varphi_{#1#1}(#2)}         % Autocorrelation function (ACF)
\newcommand{\AKFsq}[2][]{\varphi^2_{#1#1}(#2)}     % ACF^2
\newcommand{\AKFvec}[1][]{\mathbf{\boldsymbol\varphi}_{#1#1}} % ACF vector
\newcommand{\AKFmat}[1][]{\mathbf{\Phi}_{#1#1}}    % ACF matrix

\newcommand{\KKF}[2][]{\varphi_{#1}(#2)}   % Crosscorrelation function (CCF)
\newcommand{\VAR}[1][]{\sigma_{#1}^2}      % Variance
\newcommand{\VAREST}[1][]{\hat{\sigma}_{#1}^2}  % geschaetzte Varianz
\newcommand{\STDDEV}[1][]{\sigma_{#1}}     % Standardabweichung
\newcommand{\PDF}[2][]{p_{#1}(#2)}         % pdf

\newcommand{\PSD}[2][]{\Phi_{#1}(#2)}      % Power spectral density (PSD)

\newcommand{\VEC}[1]{\mathbf{#1}}          % Vector
\newcommand{\VECG}[1]{\boldsymbol{#1}}     % Vector with Greek letter
\newcommand{\MAT}[1]{\mathbf{#1}}          % Matrix
\newcommand{\MATG}[1]{\boldsymbol{#1}}     % Matrix with Greek letter

\newcommand{\LTP}[1]{\overline{#1}}        % LTP variable (as opposed to LP variable)

\newcommand{\GAUSS}{{\cal N}}              % Gaussian distribution


%%%%Integrale: El Abed-----------------------------------------------------------
\newcommand{\huellenint}{\int\!\!\!\!\!\int\limits_{\!\!\!\! A}\!\!\!\!\!\!\!\! \bigcirc \:}
\newcommand{\circint}{\int\limits_C \!\!\!\!\!\!\! \bigcirc \:}
\newcommand{\flaechenint}{\int\!\!\!\int\limits_{\!\!\!\!\!\!\! A}}


% Anordnen von Indizes usw. unter einer Funktion: ------------------------------
\newcommand{\putindex}[3]{\vtop{\hbox{\hspace{#3} $#1$}
            \hbox{\raise 6mm \hbox{$\scriptscriptstyle #2$}}}}


% Gradient von x, y, allgemein: ------------------------------------------------
\newcommand{\gradx}[0]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{\rm \hspace{2mm} \footnotesize x}}}}

\newcommand{\grady}[0]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{\rm \hspace{2mm} \footnotesize y}}}}

\newcommand{\grad}[1]{\vtop{\hbox{\rm grad}
            \hbox{\raise 2.5mm \hbox{#1}}}}


% Die Menge der reellen Zahlen: ------------------------------------------------
% \newcommand{\R}{\parbox[b]{2.4ex}{{\rm I}\hspace{-0.6ex}{\bf R}}}
% \newcommand{\Rclassic}{\parbox[b]{2.3ex}{{\rm I}\hspace{-0.6ex}{\bf R}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}

% Real- und Imaginärteil: ------------------------------------------------------
\newcommand{\real}[1]{{\rm Re}\{#1\}}
\newcommand{\imag}[1]{{\rm Im}\{#1\}}
\newcommand{\realnoarg}{{\rm Re}}
\newcommand{\imagnoarg}{{\rm Im}}

\newcommand{\comp}[1]{\underline{#1}}
\newcommand{\rect}[1]{{\rm rect}(#1)}
\newcommand{\sinc}[1]{{\rm si}(#1)}

% System T{}: ------------------------------------------------------
\newcommand{\SYSTEM}[1]{\mathfrak{T}\{#1\}}
\newcommand{\INVSYSTEM}[1]{\mathfrak{T}^{-1}\{#1\}}

% Fouriertransformation: -------------------------------------------------------
\newcommand{\invfourier}[0]{\bullet \hspace{-1.7mm} - \hspace{-1.7mm} \circ}
\newcommand{\fourier}[0]{\circ \hspace{-1.7mm} - \hspace{-1.7mm} \bullet}
%\newcommand{\FT}[1]{\mathfrak{F}\{#1\}}
\newcommand{\DTFT}[1]{{\rm DTFT}\{#1\}}
\newcommand{\DFT}[1]{{\rm DFT}\{#1\}}
\newcommand{\DCT}[1]{{\rm DCT}\{#1\}}
\newcommand{\ZT}[1]{\mathfrak{Z}\{#1\}}
\newcommand{\ZTone}[1]{\mathfrak{Z}_1\{#1\}}
\newcommand{\LT}[1]{\mathfrak{L}\{#1\}}
\newcommand{\IFT}[1]{\mathfrak{F}^{-1}\{#1\}}
\newcommand{\IDTFT}[1]{{\rm IDTFT}\{#1\}}
\newcommand{\IDFT}[1]{{\rm IDFT}\{#1\}}
\newcommand{\IDCT}[1]{{\rm IDCT}\{#1\}}
\newcommand{\IZT}[1]{\mathfrak{Z}^{-1}\{#1\}}
\newcommand{\IZTone}[1]{\mathfrak{Z}_1^{-1}\{#1\}}
\newcommand{\ILT}[1]{\mathfrak{L}^{-1}\{#1\}}

% Neue Theoremarten: -----------------------------------------------------------
%\newtheorem{definition}{Definition}[chapter]    % report, book
\newtheorem{Adefinition}{Definition}[section]   % article => A
%\newtheorem{satz}{Satz}[chapter]
%\newtheorem{ASatz}{Satz}[section]              % Be careful! TeX capacity exc.!
%\newtheorem{beweis}[satz]{Bew.:}
%\newtheorem{Abeweis}[Asatz]{Bew.:}


% Schriftgroessen: (sinnvoll in Matrizen u.a.) ---------------------------------
\newcommand{\bSs}{\scriptstyle}
\newcommand{\bSS}{\scriptscriptstyle}


% Numerierung mittels Ziffer im Kreis: -----------------------------------------
\newcommand{\ONE}{   ${\textstyle 1}\hspace{-3.2mm} \bigcirc$ }
\newcommand{\TWO}{   ${\textstyle 2}\hspace{-3.2mm} \bigcirc$ }
\newcommand{\THREE}{ ${\textstyle 3}\hspace{-3.2mm} \bigcirc$ }


% Bezeichnung von Groessen in der Diss: Patchen der Variablen im Mathemodus: --
\newcommand{\RB}[1]{#1'}             % bipolarer, BPSK-modulierter Empfangswert

\newcommand{\HB}[2][]{\hat{#2}_{#1}}           % bipolares Hardbit
\newcommand{\HBT}[2][]{{#2}_{#1}}              % bipolares Hardbit (transmitted
\newcommand{\HBR}[2][]{\hat{#2}_{#1}}          % bipolares Hardbit (received)
%\newcommand{\HBENC}[2][]{{#2}_{#1}}           % bipolares Hardbit (Sender)
\newcommand{\HBUNI}[2][]{\bar{#2}_{#1}}        % unipolares Hardbit
\newcommand{\HV}[2][]{{\underline{\hat{#2}}_{#1}}} % Vektor bipolarer Hardbits
                                               % (Parameter) (received)
\newcommand{\HVT}[2][]{{\underline{#2}_{#1}}}  % Vektor (bipolarer) Hardbits
                                               % (Parameter) (transmitted)
\newcommand{\HVTEST}[2][]{{\underline{#2}_{#1}^{\rm (est)}}} % Vektor
                                               % geschaetzter Hardbits
\newcommand{\HVR}[2][]{{\underline{\hat{#2}}_{#1}}} % Vektor
                                                    % bipolarer Hardbits
                                               % (Parameter) (received)
%\newcommand{\HVENC}[2][]{{\bf{#2}_{#1}}}      % Vektor (bipolarer) Hardbits
                                               % (Sender)

\newcommand{\SB}[2][]{\tilde{#2}_{#1}}         % bipolares Softbit
\newcommand{\CORR}[2][]{\tilde{#2}_{#1}}       % bipolares Softbit
\newcommand{\SBUNI}[2][]{\breve{#2}_{#1}}      % unipolares Softbit
\newcommand{\SV}[2][]{{\underline{\tilde{#2}}_{#1}}} %Vektor bipolarer Softbits

\newcommand{\EST}[2][]{{#2}_{#1}^{\rm (est)}}  % geschaetzter Parameter
\newcommand{\MS}[2][]{{#2}_{#1}^{\rm (MS)}}    % MS-geschaetzter Parameter,fett
\newcommand{\VARMS}[2][]{{#2}_{#1}^{\rm (MS)}} % MS-geschaetzter Parameter
\newcommand{\MEAN}[2][]{{#2}_{#1}^{\rm (MEAN)}} % Mean-geschaetzter Par.
\newcommand{\MAP}[2][]{{#2}_{#1}^{\rm (MAP)}}  % MAP-geschaetzter Par.
\newcommand{\ML}[2][]{{#2}_{#1}^{\rm (ML)}}    % MAP-geschaetzter Par.
\newcommand{\VAROK}[2][]{{#2}_{#1}^{\rm (OK)}} % ungestoerter Parameter
%\newcommand{\MS}[2][]{{#2}_{{#1}_{\rm MS}}}   % MS-geschaetzter Parameter,fett
%\newcommand{\VARMS}[2][]{{#2}_{{#1}_{\rm MS}}} % MS-geschaetzter Parameter
%\newcommand{\MEAN}[2][]{{#2}_{{#1}_{\rm M}}}   % Mean-geschaetzter Par.
%\newcommand{\MAP}[2][]{{#2}_{{#1}_{\rm MAP}}}  % MAP-geschaetzter Par.
%\newcommand{\ML}[2][]{{#2}_{{#1}_{\rm ML}}}    % MAP-geschaetzter Par.
%\newcommand{\VAROK}[2][]{{#2}_{{#1}_{\rm OK}}} % ungestoerter Parameter
%\newcommand{\VECold}[2][]{{#2}_{#1}}             % Vektor, Parameter (allgemein)
\newcommand{\PART}[2][]{{\tilde{#2}_{#1}}}     % unquantisierter Parameter
                                               % (Transmitter)
\newcommand{\QPART}[2][]{{#2}_{#1}}            % quantisierter Parameter
                                               % (transmitted)
\newcommand{\QPARR}[2][]{{\hat{#2}_{#1}}}      % quantisierter Parameter
                                               % (received)
\newcommand{\PAREST}[2][]{{\tilde{#2}^{\rm (est)}_{#1}}}%geschaetzter Parameter
                                               % (received)

\newcommand{\VARBER}[1][]{{p^{(#1)}_e}}    % momentane, gemessene Bitfehlerrat
\newcommand{\BER}[1][]{{p_{e#1}}}          % momentane, gemessene Bitfehlerrate

\newcommand{\PROBD}[1][]{{\rm p_{#1}}}         % p( ),Wahrscheinlichkeitsdichte
\newcommand{\PROB}[0]{{\rm P}}        % P( ),   Wahrscheinlichkeit
\newcommand{\VARPROB}[0]{{\rm Prob}}  % Prob(), Wahrscheinlichkeit

%\newcommand{\QUANTINV}[1]{{\bf Q^{-1}[}#1{\bf ]}} % Inverse Qu.funktion
\newcommand{\BMINV}[1]{{\bf BM^{-1}[}#1{\bf ]}}   % Inverses Bit-Mapping
\newcommand{\BM}[1]{{\bf BM[}#1{\bf ]}}   % Inverses Bit-Mapping



\newcommand{\EV}[1]{E\{{#1}\}}                    % Erwartungswert
\newcommand{\EVEST}[1]{\hat{E}\{{#1}\}}           % geschaetzter Erwartungswert

%\newcommand{\Dist}{\tilde{D}}
\newcommand{\AKFold}[1]{R_{#1 #1}}               % Autokorrelationsfunktion
\newcommand{\AKFEST}[1]{\hat{R}_{#1 #1}}      % geschaetzter AKF-Wert
\newcommand{\ACOVF}[1]{C_{#1 #1}}             % Autocovarianzfunktion
\newcommand{\AKCOEF}[1]{\rho_{#1 #1}}         % (Auto-) Korrelationskoeffizient
\newcommand{\RHO}[0]{\rho}                    % 1. Auto-Korrelationskoeffizient
\newcommand{\AKCOEFEST}[1]{\hat{\rho}_{#1 #1}} % geschaetzter Korr.-koeffizient
\newcommand{\MW}[1]{\eta_{#1}}                % Mittelwert
\newcommand{\MWEST}[1]{\hat{\eta}_{#1}}       % geschaetzter Mittelwert
\newcommand{\KKFold}[2]{R_{#1 #2}}               % Kreuzkorrelationsfunktion
\newcommand{\KKCOEF}[2]{\rho_{#1 #2}}         % Kreuzkorrelationskoeffizient
\newcommand{\LDSP}[1]{\Phi_{#1 #1}}           % Leistungsdichtespektrum
\newcommand{\SFM}[0]{\gamma}                  % spektrales Flachheitsmass
\newcommand{\SD}[0]{{\rm SD}}                 % spektraler Abstand

\newcommand{\VARLB}[1][]{L_{#1}}              % L-Wert ohne Bitkomb.-Bez.nung
\newcommand{\LB}[2][]{L^{(#2)}_{#1}}               % L-Wert
\newcommand{\LV}[2][]{{\underline{L}^{(#2)}_{#1}}} % Vektor L-Werte

\newcommand{\DRtheo}[0]{\Delta R}             % theoretische Redundanz
\newcommand{\DRVtheo}[0]{\Delta R_{\rm v}}    % th. verteilungsabhaengige Red.
\newcommand{\DRKtheo}[0]{\Delta R_{\rm k}}    % th. korrelationsabh"angige Red.
\newcommand{\DR}[0]{\Delta R'}                % nutzbare Redundanz
\newcommand{\DRV}[0]{\Delta R_{\rm v}'}       % nb. verteilungsabhaengige Red.
\newcommand{\DRK}[0]{\Delta R_{\rm k}'}       % nb. korrelationsabh"angige Red.
\newcommand{\RBRUTTO}[0]{R_{\rm brutto}}      % Bruttobitrate
\newcommand{\RCHCOD}[0]{R_{\rm CHCOD}}        % Nettobitrate CHCOD
\newcommand{\RSD}[0]{R_{\rm SD}}              % Nettobitrate SD
\newcommand{\DRCHCOD}[0]{\Delta R_{\rm CHCOD}} % Redundanz durch Kanalcod. (r)
\newcommand{\GPtheo}[0]{G_p}                  % theoretischer Praedikt.Gewinn
\newcommand{\GP}[0]{G_p'}                     % real erreichter Praedikt.Gewinn
\newcommand{\NGD}[0]{\epsilon}                % Nutzungsgrad der Redundanz
\newcommand{\NGV}[0]{\epsilon_{\rm v}}        % ... der verteilungsabh. Red.
\newcommand{\NGK}[0]{\epsilon_{\rm k}}        % ... korrelationsabh. Red.
\newcommand{\DRVLMQ}[0]{\Delta R_{\rm v (LMQ)}'}  % nb. vert.abh. Red. des LMQ
\newcommand{\DRVMEQ}[0]{\Delta R_{\rm v (MEQ)}'}  % nb. vert.abh. Red. des MEQ


\newcommand{\ARN}[0]{\bar{N}}                 % echte AR-Ordnung eines Par's

\newcommand{\FA}[0]{f_A}                      % Abtastfrequenz

\newcommand{\CHF}[1]{{\rm \Psi_{#1}}}         % Charakteristische Funktion


%==============================================================================
% Hier folgen Macros, die zwar nicht mathematischer Natur sind, jedoch
% in texten haeufig gebraucht werden.


% Symmetrische Zeileneinstellung fuer Tabellen (Stuetze): ---------------------
\newcommand{\stz}{\rule{0mm}{2.3ex}}
\newcommand{\stzsym}{\rule[-0.8ex]{0mm}{3.1ex}}
\newcommand{\stzdown}{\rule[-1.2ex]{0mm}{3.5ex}}
\newcommand{\stzlargesym}{\rule[-1.8ex]{0mm}{5.1ex}}

% Abkuerzung fuer die Tabulator-Umgebung: -------------------------------------
\newcommand{\btb}{     \begin{tabbing}             }
\newcommand{\bte}{     \end{tabbing}               }

==> tab/tu_bs_colors.tex <==
\definecolor{tu0}{rgb}{0.7451, 0.1176, 0.2353}

\definecolor{tu1}{rgb}{1.0000, 0.8039, 0.0000}
\definecolor{tu11}{rgb}{1.0000, 0.8627, 0.3020}
\definecolor{tu12}{rgb}{1.0000, 0.9020, 0.4980}
\definecolor{tu13}{rgb}{1.0000, 0.9412, 0.6980}
\definecolor{tu14}{rgb}{1.0000, 0.9608, 0.8000}

\definecolor{tu2}{rgb}{0.9804, 0.4314, 0.0000}
\definecolor{tu21}{rgb}{0.9882, 0.6039, 0.3020}
\definecolor{tu22}{rgb}{0.9882, 0.7137, 0.4980}
\definecolor{tu23}{rgb}{0.9922, 0.8275, 0.6980}
\definecolor{tu24}{rgb}{0.9961, 0.8863, 0.8000}

\definecolor{tu3}{rgb}{0.6902, 0.0000, 0.2745}
\definecolor{tu31}{rgb}{0.7529, 0.2000, 0.4196}
\definecolor{tu32}{rgb}{0.8431, 0.4980, 0.6353}
\definecolor{tu33}{rgb}{0.9216, 0.7490, 0.8196}
\definecolor{tu34}{rgb}{0.9529, 0.8510, 0.8902}

\definecolor{tu4}{rgb}{0.4863, 0.8039, 0.9020}
\definecolor{tu41}{rgb}{0.6431, 0.8627, 0.9333}
\definecolor{tu42}{rgb}{0.7412, 0.9020, 0.9490}
\definecolor{tu43}{rgb}{0.8431, 0.9412, 0.9686}
\definecolor{tu44}{rgb}{0.8980, 0.9608, 0.9804}

\definecolor{tu5}{rgb}{0.0000, 0.5020, 0.7059}
\definecolor{tu51}{rgb}{0.3020, 0.6510, 0.7961}
\definecolor{tu52}{rgb}{0.5490, 0.7765, 0.8667}
\definecolor{tu53}{rgb}{0.7490, 0.8745, 0.9255}
\definecolor{tu54}{rgb}{0.8510, 0.9255, 0.9569}

\definecolor{tu6}{rgb}{0.0000, 0.3255, 0.4549}
\definecolor{tu61}{rgb}{0.2510, 0.4941, 0.5922}
\definecolor{tu62}{rgb}{0.5490, 0.6941, 0.7529}
\definecolor{tu63}{rgb}{0.7490, 0.8314, 0.8627}
\definecolor{tu64}{rgb}{0.8510, 0.8980, 0.9176}

\definecolor{tu7}{rgb}{0.0314, 0.0314, 0.0314}
\definecolor{tu71}{rgb}{0.3725, 0.3725, 0.3725}
\definecolor{tu72}{rgb}{0.5882, 0.5882, 0.5882}
\definecolor{tu73}{rgb}{0.7529, 0.7529, 0.7529}
\definecolor{tu74}{rgb}{0.8667, 0.8667, 0.8667}

\definecolor{tu8}{rgb}{0.7765, 0.9333, 0.0000}
\definecolor{tu81}{rgb}{0.8431, 0.9529, 0.3020}
\definecolor{tu82}{rgb}{0.8863, 0.9647, 0.4980}
\definecolor{tu83}{rgb}{0.9333, 0.9804, 0.6980}
\definecolor{tu84}{rgb}{0.9569, 0.9882, 0.8000}

\definecolor{tu9}{rgb}{0.5373, 0.6431, 0.0000}
\definecolor{tu91}{rgb}{0.6784, 0.7490, 0.3020}
\definecolor{tu92}{rgb}{0.7686, 0.8196, 0.4980}
\definecolor{tu93}{rgb}{0.8588, 0.8941, 0.6980}
\definecolor{tu94}{rgb}{0.9059, 0.9294, 0.8000}

\definecolor{tu10}{rgb}{0.0000, 0.4431, 0.3373}
\definecolor{tu101}{rgb}{0.3020, 0.6118, 0.5373}
\definecolor{tu102}{rgb}{0.5490, 0.7490, 0.7020}
\definecolor{tu103}{rgb}{0.7490, 0.8588, 0.8353}
\definecolor{tu104}{rgb}{0.8549, 0.9176, 0.9059}

\definecolor{tu110}{rgb}{0.8000, 0.0000, 0.6000}
\definecolor{tu111}{rgb}{0.8706, 0.3490, 0.7412}
\definecolor{tu112}{rgb}{0.9216, 0.6000, 0.8392}
\definecolor{tu113}{rgb}{0.9608, 0.8000, 0.9216}
\definecolor{tu114}{rgb}{0.9804, 0.8980, 0.9608}

\definecolor{tu120}{rgb}{0.4627, 0.0000, 0.4627}
\definecolor{tu121}{rgb}{0.5961, 0.2510, 0.5961}
\definecolor{tu122}{rgb}{0.7294, 0.4980, 0.7294}
\definecolor{tu123}{rgb}{0.8392, 0.6980, 0.8392}
\definecolor{tu124}{rgb}{0.9216, 0.8510, 0.9216}

\definecolor{tu130}{rgb}{0.4627, 0.0000, 0.3294}
\definecolor{tu131}{rgb}{0.6118, 0.3020, 0.5333}
\definecolor{tu132}{rgb}{0.7569, 0.5490, 0.6980}
\definecolor{tu133}{rgb}{0.8667, 0.7490, 0.8314}
\definecolor{tu134}{rgb}{0.9216, 0.8510, 0.9020}

==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
%
%
% Modifications 2017 by Tycho Groche
%
% -------------------------------------------------------------------------

\usetikzlibrary{arrows,
	calc,
	positioning,
	decorations.markings,
	shapes,
	decorations}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter


\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }

	  \foreach \x in {center, mid, mid west, mid east, base, base west, base east,
	  	north, north east, east, south east, south, south west, west, north west}{
	  	\inheritanchor[from={circle}]{\x}
	  }
	  \inheritanchorborder[from={circle}]

	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}

	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }

		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima

	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}

	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima

	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}

	\pgfusepathqstroke
}

\pgfdeclareshape{dspshapesaturation}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}
		\pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\southwest}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
	}
}


\pgfdeclareshape{dspshapelowpass}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		%coordinate system
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa} {0.33\pgf@ya}}
		%lowpass
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.2\pgf@xa} {0.33\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapebandpass}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		%coordinate system
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa} {0.33\pgf@ya}}
		%lowpass
		\pgfpathmoveto{\pgfpoint{0.15\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.1\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.1\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa} {0.33\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapesinewave}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast

		\pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}

		\pgfpathmoveto{\pgfpoint{0.3\pgf@xa}{0}}
		\pgfpathsine{\pgfpoint{-0.15\pgf@xa}{0.25\pgf@ya}}
		\pgfpathcosine{\pgfpoint{-0.15\pgf@xa}{-0.25\pgf@ya}}
		\pgfpathsine{\pgfpoint{-0.15\pgf@xa}{-0.25\pgf@ya}}
		\pgfpathcosine{\pgfpoint{-0.15\pgf@xa}{0.25\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapepulse}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast

		\pgfpathmoveto{\pgfpoint{0.3\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@xa}{-0.15\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa}{-0.15\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.3\pgf@xa}{0.2\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapeadaptive}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{arrowstart}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\southwest
		\advance\pgf@x by -0.05\pgf@xa
		\advance\pgf@y by 0.3\pgf@ya
	}

	\anchor{arrowend}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\advance\pgf@x by 0.05\pgf@xa
		\advance\pgf@y by -0.3\pgf@ya
	}

	\behindbackgroundpath
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y

		\southwest
		\advance\pgf@x by -0.05\pgf@xa
		\advance\pgf@y by 0.3\pgf@ya
		\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}

		\northeast
		\advance\pgf@x by 0.05\pgf@xa
		\advance\pgf@y by -0.3\pgf@ya

		\pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
		\pgfsetarrowsend{latex}
		\pgfsetlinewidth{\dsplinewidth}
		\pgfsetroundcap
		\pgfusepath{stroke}
	}

	\beforebackgroundpath
	{
    	\pgfpathrectanglecorners
		{\pgfpointadd{\southwest}{\pgfpoint{\dspblocklinewidth}{\dspblocklinewidth}}}
		{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\dspblocklinewidth}{\dspblocklinewidth}}}}

		\color{white}
		\pgfusepath{fill}
	}


}


\pgfdeclareshape{dspshapefourpole}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{west top}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\southwest}
		\advance\pgf@y by -0.85\pgf@ya
	}

	\anchor{west bottom}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\southwest}
		\advance\pgf@y by -0.15\pgf@ya
	}

	\anchor{east top}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\northeast}
		\advance\pgf@y by 0.15\pgf@ya
	}

	\anchor{east bottom}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\northeast}
		\advance\pgf@y by 0.85\pgf@ya
	}
}


\pgfdeclareshape{dspshapemic}{

	\inheritsavedanchors[from={circle}]
	\inheritbackgroundpath[from={circle}]
	\inheritanchorborder[from={circle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}	{
		\inheritanchor[from={circle}]{\x}
	}


	\beforebackgroundpath{
	\pgfmathsetlength\pgf@xa{\radius}

	\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@xa}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{-\pgf@xa}}

	\pgfusepathqstroke
	}
}


\pgfdeclareshape{dspshapespeaker}{

	\inheritsavedanchors[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{speaker}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\advance\pgf@x by -\pgf@xa
		\advance\pgf@y by 0.5\pgf@ya
	}

	\backgroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y

		\pgfpathmoveto{\northeast}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-\pgf@xc}{-0.5\pgf@yc}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-\pgf@xc}{1.5\pgf@yc}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{0}{1\pgf@yc}}}

		\pgfpathrectanglecorners{\southwest}{\northeast}

	}

}

% -------------------------------------------------------------------------
% Decoration for corner-aligned dashed border
%--------------------------------------------------------------------------
%https://tex.stackexchange.com/questions/280187/create-corner-aligned-dashed-rectangles-using-tikz

\def\pgf@dec@dashon{5pt}
\def\pgf@dec@dashoff{5pt}
\pgfkeys{/pgf/decoration/.cd,
	/pgf/decoration/dash on/.store in=\pgf@dec@dashon,
	/pgf/decoration/dash off/.store in=\pgf@dec@dashoff
}
\pgfdeclaredecoration{aligned dash}{start}{
	\state{start}[width=0pt, next state=pre-corner,persistent precomputation={
		\pgfextract@process\pgffirstpoint{\pgfpointdecoratedinputsegmentfirst}%
		\pgfextract@process\pgfsecondpoint{\pgfpointdecoratedinputsegmentlast}%
		\pgfmathsetlengthmacro\pgf@dec@dashon{\pgf@dec@dashon}%
		\pgfmathsetlengthmacro\pgf@dec@dashoff{\pgf@dec@dashoff}%
		\pgfmathsetlengthmacro\pgf@dec@halfdash{\pgf@dec@dashon/2}%
	}]{}
	\state{pre-corner}[width=\pgfdecoratedinputsegmentlength, next state=post-corner, persistent precomputation={
		%
		\pgfmathparse{int(ceil((\pgfdecoratedinputsegmentlength-\pgf@dec@dashon-\pgf@dec@dashoff)/(\pgf@dec@dashon+\pgf@dec@dashoff)))}%
		\let\pgf@n=\pgfmathresult
		\pgfmathsetlengthmacro\pgf@b%
		{\pgfdecoratedinputsegmentlength/(\pgf@n+1)-\pgf@dec@dashon}%
		\ifdim\pgf@b<\pgf@dec@dashoff\relax%
		\pgfmathparse{int(\pgf@n-1)}\let\pgf@n=\pgfmathresult%
		\pgfmathsetlengthmacro\pgf@b%
		{\pgfdecoratedinputsegmentlength/(\pgf@n+1)-\pgf@dec@dashon}%
		\fi%
		\pgfmathsetlengthmacro\pgf@b{\pgf@b+\pgf@dec@dashon}%
	}]{%
		\pgfmathloop
		\ifnum\pgfmathcounter>\pgf@n%
		\else%
		\pgfpathmoveto{\pgfpoint{\pgf@b*\pgfmathcounter-\pgf@dec@halfdash}{0pt}}%
		\pgfpathlineto{\pgfpoint{\pgf@b*\pgfmathcounter+\pgf@dec@halfdash}{0pt}}%
		\repeatpgfmathloop%
		\pgfpathmoveto%
		{\pgfpoint{\pgfdecoratedinputsegmentlength-\pgf@dec@halfdash}{0pt}}%
		\pgfpathlineto%
		{\pgfpointdecoratedinputsegmentlast}
	}
	\state{post-corner}[width=0pt, next state=pre-corner]{
		\pgfpathlineto{\pgfpoint{\pgf@dec@halfdash}{0pt}}%
	}
	\state{final}{
		\pgftransformreset%
		\pgfpathlineto{\pgfpointlineatdistance{\pgf@dec@halfdash}{\pgffirstpoint}{\pgfsecondpoint}}%
	}
}


\makeatother

% -------------------------------------------------------------------------
% Define border styles
%--------------------------------------------------------------------------

\tikzset{aligned dash/.style=
	{
		decoration=
		{
			aligned dash,
			#1
		},
		decorate
	}
}


% -------------------------------------------------------------------------
% Define node styles
%--------------------------------------------------------------------------

\tikzset{dspadder/.style=
	{
		shape=dspshapeadder,
		line cap=rect,
		line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspmultiplier/.style=
	{
		shape=dspshapecircle,
		line cap=rect
		,line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspmixer/.style=
	{
		shape=dspshapemixer,
		line cap=rect,
		line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspnodeopen/.style=
	{
		shape=dspshapecircle,
		line width=\dsplinewidth,
		minimum size=\dspnoderadius
	}
}


\tikzset{dspnodefull/.style=
	{
		shape=dspshapecirclefull,
		line width=\dsplinewidth,
		fill,
		minimum size=\dspnoderadius
	}
}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style=
	{
		shape=rectangle,
		draw,
		align=center,
		text depth=0.3em,
		text height=1em,
		inner sep=0pt,
		line cap=round,
		line join=round,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspfilter/.style=
	{
		shape=rectangle,
		draw,
		align=center,
		text depth=0.3em,
		text height=1em,
		inner sep=0pt,
		line cap=round,
		line join=round,
		line width=\dsplinewidth,
		minimum height=\dspsquareblocksize,
		minimum width=\dspfilterwidth
	}
}


\tikzset{dspgain/.style=
	{
		draw,
		isosceles triangle,
		isosceles triangle apex angle=60,
		minimum width = \dspsquareblocksize,
		inner sep = 0pt
	}
}


\tikzset{dspsaturate/.style=
	{
		draw,
		shape=dspshapesaturation,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspsinewave/.style=
	{
		draw,
		shape=dspshapesinewave,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dsppulse/.style=
	{
		draw,
		shape=dspshapepulse,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dsplowpass/.style=
	{
		draw,
		shape=dspshapelowpass,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspbandpass/.style=
	{
		draw,
		shape=dspshapebandpass,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspadaptivefilter/.style=
	{
		draw,
		shape=dspshapeadaptive,
		line width=\dspblocklinewidth,
		minimum height = \dspsquareblocksize,
		minimum width=\dspfilterwidth
	}
}


\tikzset{dspsystem/.style=
	{
		draw,
		line width = 0.5*\dspblocklinewidth,
		inner sep = 10pt,
		aligned dash =
		{
			%
		}
	}
}


\tikzset{dspmic/.style=
	{
		draw,
		shape = dspshapemic,
		line width = \dspblocklinewidth,
		minimum size = \dspoperatordiameter
	}
}


\tikzset{dspspeaker/.style=
	{
		draw,
		shape = dspshapespeaker,
		line width = \dspblocklinewidth,
	}
}


\tikzset{dspfourpole/.style=
	{
		draw,
		shape = dspshapefourpole,
		inner sep = 0cm,
		line width = \dspblocklinewidth,
		minimum size = 2.6*\dspsquareblocksize
	}
}


% -------------------------------------------------------------------------
% Define "signal flow" lines
%--------------------------------------------------------------------------

\tikzset{dspline/.style=
	{
		line width=\dsplinewidth
	},
	line cap=round,
	line join=round
}


\tikzset{dspconn/.style=
	{
		->,
		>=dsparrow,
		line width=\dsplinewidth
	},
	line cap=round,
	line join=round
}


\tikzset{dspflow/.style=
	{
		line width=\dsplinewidth,
		line cap=round,
		line join=round,
		decoration=
		{
			markings,
			mark=at position 0.5 with
			{
				\arrow{dsparrowmid}
			}
		},
		postaction={decorate}
	}
}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

